Sleeper Agent: Scalable Hidden Trigger Backdoors for Neural Networks Trained from Scratch

As the curation of data for machine learning becomes increasingly automated, dataset tampering is a mounting threat. Backdoor attackers tamper with training data to embed a vulnerability in models that are trained on that data. This vulnerability is then activated at inference time by placing a "trigger" into the model's input. Typical backdoor attacks insert the trigger directly into the training data, although the presence of such an attack may be visible upon inspection. In contrast, the Hidden Trigger Backdoor Attack achieves poisoning without placing a trigger into the training data at all. However, this hidden trigger attack is ineffective at poisoning neural networks trained from scratch. We develop a new hidden trigger attack, Sleeper Agent, which employs gradient matching, data selection, and target model re-training during the crafting process. Sleeper Agent is the first hidden trigger backdoor attack to be effective against neural networks trained from scratch. We demonstrate its effectiveness on ImageNet and in black-box settings. Our implementation code can be found at https://github.com/hsouri/Sleeper-Agent.

==> checklist.tex <==
\newpage


\section*{Checklist}



\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:br_lim}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec:br_lim}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{app:imp_det}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{app:imp_det}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We defer to licenses on the respective host websites for the datasets we use. We use assets for purely research reasons.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See supplementary material}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> limitations.tex <==
\section{Limitations}
\label{sec:limits}
% In this work, we propose an attack that has the potential to have pernicious applications. An attacker could employ a method like ours in order to maliciously control deep networks of unsuspecting victims. While there has been application of data poisoning techniques to important tasks like watermarking for intellectual property protection \cite{uchida2017embedding}, the more apparent application of our method is an attack. However, we believe that investigating and publishing information about attacks is important for revealing security vulnerabilities in mainstream models.  We hope that our work consequently inspires the development of improved defenses.

% While our attack vastly outperforms existing methods on from-scratch backdoor poisoning, it does still have limitations which warrant future investigation. First is the need to access a pretrained model in order to estimate the training and adversarial gradient in Equation \ref{eq:align}. This may not be realistic for an attacker who has partial knowledge of the data/labels that a victim is using. %This is, however, a limitation that exists in Hidden Trigger Backdoors which requires access to the \emph{exact} pretrained feature extractor used by the victim in order for the attack to successfully cause feature collision.
% Second is the instability that arises from choosing different source and target class pairs. While on average our method works quite well, the variance is large, and the success of our method can range from almost all patched images being misclassified to low success. This behavior has previously been observed in \cite{schwarzschild2020just}.  In real-world scenarios, datasets are often noisy and imbalanced, so training behavior may be mysterious.  As a result, practitioners should be cautious in their expectations that methods developed on datasets like CIFAR-10 and ImageNet will work on their own problems.


While on average, our method is effective, the variance is large, and the success of our method can range from almost all patched images being misclassified to low success. This behavior has previously been observed in \cite{schwarzschild2020just}.  In real-world scenarios, datasets are often noisy and imbalanced, so training behavior may be mysterious.  As a result, practitioners should be cautious in their expectations that methods developed on datasets like CIFAR-10 and ImageNet will work on their own problems.


==> societal_impact.tex <==
\section{Potential Negative Societal Impact}

In this work, we illuminate a new scalable backdoor attack that could be used to stealthily compromise security-critical systems.  We hope that by highlighting the potential danger of this nefarious threat model, our work will give rise to stronger defenses and will encourage caution on the part of practitioners.
